PEDANTS: Cheap but Effective and Interpretable Answer Equivalence

Question answering (QA) can only make progress if we know if an answer is correct, but current answer correctness (AC) metrics struggle with verbose, free-form answers from large language models (LLMs). There are two challenges with current short-form QA evaluations: a lack of diverse styles of evaluation data and an over-reliance on expensive and slow LLMs. LLM-based scorers correlate better with humans, but this expensive task has only been tested on limited QA datasets. We rectify these issues by providing rubrics and datasets for evaluating machine QA adopted from the Trivia community. We also propose an efficient, and interpretable QA evaluation that is more stable than an exact match and neural methods(BERTScore).

==> sections/20-error-analysis.tex <==
\section{Motivation}
\label{sec:limitations}

% \jbgcomment{I think this section would be stronger if:

%   - you had a roadmap at the begining talking about what this section will be about: reviewing \equivalence{}, error analysis, how that leads to a conclusion that OOD generalization is lacking

%   - you need to make the case to reviewers that exact match isn't enough.  you're deep into the weeds on this, but you're likely going to get a reviewer who uses exact match and doesn't see the problem.  Get them to see the problems!

%   - I think you spend too much time on BEM.  This is a paper about what you did, so don't focus too much on them.  Perhaps just cite them, ignore their annotations (for now anyway), and just focus on applying their AE to the dataset.  You can contrast how their annotations are different from yours later.

% }
% \ishanicomment{Maybe, we should clearly demarcate and create a table saying that the existing datasets, evaluation metrics capture these aspects, while our metric can handle something else... Look at Table 9 https://openreview.net/pdf?id=4dsMX3RnF0. Give examples from various datasets (Six datasets) highlighting the potential concerns that can't be captured in earlier metrics or even GPT-4Eval}
% \zongxiacomment{There is a table in the appendix}

% This section reviews the current state and definition of \abr{qa} evaluations.
%
This section analyzes limitations of the popular \abr{qa} evaluation
methods---\abr{em}, token $F_1$, \bertscore{}~\cite{Zhang2019BERTScoreET},
\abr{bem}~\cite{bulian2022tomayto}, \abr{lerc}~\cite{Chen_2020}---on Reading Comprehension with Commonsense
Reasoning~\cite{lin-etal-2019-reasoning} \textit{dev} set.
% and we show the pitfalls of
% current evaluation methods. We specifically present annotated examples in Section~\ref{section:generalization}
% to show the lack of generalization of these evaluation methods on
% out-of-distribution (\abr{ood}) datasets. especially for
% \abr{bert}-based methods trained on \ac{} data generated only from
% the Stanford Question Answering Dataset~\cite{rajpurkar2016squad}.

% \begin{table}[ht]
% \small
% \centering
% \begin{tabular}{ccccc}
% \hline
% Metric($\%$) & \abr{em} & \abr{bem} & RoBERTa & LLAMA 2 \\ \hline
% dev  & 49.96   & 89.39 & 90.11 & 91.54  \\
% test & 54.74   & 89.96  & 90.11 & 90.43 \\ \hline
% \end{tabular}
% \caption{The accuracy on \abr{em} and \abr{bem}, RoBERTA, and LLAMA 2 aligns with human judgments on the \ac{} dev and test set. \abr{em} significantly misaligns with human judgments on correctness}
% \label{tab: google-ae-accuracy}
% \end{table}

% \begin{table*}[ht]
% \centering
% \begin{tabular}{m{0.13\textwidth} m{0.08\textwidth} m{0.37\textwidth} m{0.16\textwidth} m{0.14\textwidth}}
% \hline
% \textbf{Dataset} & \textbf{\# Pairs} & \textbf{Context} & \textbf{Question} & \textbf{Gold Answer} \\ \hline
% \abr{nq-open} & 3,610 & \multicolumn{1}{c}{-} & who won the American league east in 2017 & The Yankees, Houston Astros \\ \hline 
% Trivia\abr{qa} & 3,313 & Asmara International Airport (IATA: ASM) (ICAO: HHAS). Asmara currently hosts the country's only operating international airport... & Asmara international airport is in which country? & Eritrea \\ \hline
% \abr{\abr{ropes}} & 1,688 & Sometimes muscles and tendons get injured ... Greg sees Carl doing some warm ups and laughs to himself and thinks it is silly ... and are both avid runners. & Who is more likely to get an injury during the race? & Greg \\ \hline
% Narrative-\abr{qa} & 3,774 & The narrator, a Bostonian, returns after a brief visit a few summers prior, to the small coastal town ... cMaine coastal town increases each day. & What was Littlepage's job? & sailor, retired sailor \\ 
% \hline
% \end{tabular}
% \caption{The 4 datasets used in our study to evaluate automated QA metrics, along with selected samples of the \textit{Question} and \textit{Gold Answer} pairs for each.}


% % \caption{Number of \abr{qa} pair examples and datasets we use in our study to evaluate automated \abr{qa} evaluation metrics. The cell with `-' indicates the \abr{qa} pairs do not have related contexts.}

% \label{tab:dataset}
% \end{table*}

% \begin{table*}[ht]
% \centering
% \begin{tabular}{p{0.13\textwidth} p{0.10\textwidth} p{0.37\textwidth} p{0.14\textwidth} p{0.14\textwidth}}
% \hline
% \textbf{Dataset} & \textbf{\# Pairs} & \textbf{Context} & \textbf{Question} & \textbf{Gold Answer} \\ \hline
% \abr{nq-open} & 3,610 & \multicolumn{1}{c}{-} & who won the American league east in 2017 & The Yankees, Houston Astros \\ 
% \abr{\abr{ropes}} & 1,688 & Sometimes muscles and tendons get injured ... Greg sees Carl doing some warm ups and laughs to himself and thinks it is silly ... and are both avid runners. & Who is more likely to get an injury during the race? & Greg \\ 
% Narrative \abr{qa} & 15,774 & Clara Amedroz is the only surviving child of the elderly squire ... can she bring herself to put aside her scruples and accept him. Marital bliss ensues. & Data 9 & Data 10 \\
% Data 6 & Data 7 & More long text in the cell that wraps around & Data 9 & Data 10 \\
% \hline
% \end{tabular}
% \caption{Your Table Caption}
% \label{tab:my_table}
% \end{table*}


% \begin{figure}
%     % \centering
%   \includegraphics[scale=0.65]{figures/demo3.pdf}
%   \jbgcomment{1.  I'm not sure this should be a figure; either make it look nicer or return to text.  :)  2.  Make sure the takeaway is the first sentence of the caption.  In this case, it's not strong enough.  E.g., ``Existing \equivalence{} methods (e.g., BEM as seen here) fail to detect\dots)}
%     \caption{We show the number of \abr{fp} and \abr{fn} for \abr{em}, $F_1$, and \abr{bem} compared to human judgments on the \abr{ropes} test set (1,688 examples). While \abr{em} the problem of being too strict, often classifies correct \can{} answers as incorrect, $F_1$ only measures token overlap without considering any semantic information. \abr{bem} significantly fails to detect correctness of a \can{} answer on an \abr{ood} dataset.}
%     \label{fig:demo}
% \end{figure}



% \subsection{Correctness Verification}
% ~\cite{bulian2022tomayto} provides basic definition of \ac{} and a dataset with human judgements to determine \ac{}, that any answers with extra important correct information should be credited, and answers omitting relevant information should be ruled incorrect. The \ac{} dataset is derived from ~\cite{rajpurkar2016squad} and includes a 9,090 train examples, 4,446 dev examples and 9,824 test examples that contains crowd-sourced human annotated judgments on answer correctness, where each example contains the context for the question, the question, a \refer{} answer, a \can{} answer, and the human judgment of the \can{} answer. We start to analyze the alignment of \abr{bem} and \abr{em} with human judgments for in-distribution data by evaluating accuracy of \abr{bem} and \abr{em} on the \ac{} dev and test set.~\footnote{We use a threthold of greater than 0.5 to judge an answer to be correct using \abr{bem} since \abr{bem} is trained with best performance with 0.5 threshold} In addition, we also trained RoBERTa-base and LLAMA 2 on the \ac{} train set as additional automated correctness evaluation models to analyze the weaknesses of the current current definition of \ac{}, the \ac{} dataset, and current automated evaluation models.~\footnote{Training details for RoBERTa-base and LLAMA 2 is in Appendix. We use LLAMA 2 with 7B parameter sizes} Table ~\ref{tab: google-ae-accuracy} shows that \abr{em} is least aligned with human correctness judgments, with \abr{bem}, RoBERTa, and LLAMA 2 that highly correlates to human judgments. Although \abr{llm}-based models show a significant correlation to human judgments for in-distribution datasets, the generalization of smaller language models on evaluating answer correctness for out of distribution (\abr{ood}) data remains an open questions for us. Our hypothesis is that \abr{bem} and RoBERTa will not generalize well for \abr{ood} data in correctness evaluation comparing with human judgments.
% \paragraph{\abr{ropes} Dataset} is designed to evaluate a model's ability to reason about cause and effect within a given text. Each example in the dataset has an associated context, a question, and a \refer{} answer. 

% \ishanicomment{I guess all of these things that we are discussing in this current QA Evaluation Limitations, can we just have a nice table with examples that I commented above and then put a link in the introduction so that the lazy reviewer can directly hover over? That should save space}
% \subsection{Current \abr{qa} evaluations}
% \label{sec:eval_methods}
%
% The definition of \ac{} varies depending on the type of evaluation
% methods. We present three \abr{qa} evaluation methods with their
% definitions, which we will also use for our error analysis in
% section~\ref{section:generalization}. 
%

% \jbgcomment{perhaps create a macro for \refer{} and \can{}s}
% \jbgcomment{don't use spaces in labels (it screws up autocomplete in Overleaf)
% }

\paragraph{Exact Match (\abr{em})}
%
We follow ~\citet{izacard2021leveraging}'s implementation, where a generated
answer is correct if it matches any of the reference answers in the list after
normalization: removing articles, duplicate white spaces, punctuation.
% It is the simplest and most-used \abr{qa}
% evaluation for its efficiency. In this case of two strings do not match, the \can{} is considered incorrect.
% \jbgcomment{style checker should have flagged ``X nature''; this can almost always be replaced by just saying that it's X}
% \abr{em} evaluates a machine \abr{qa} system's ability to
% produce an answer that exactly matches an answer in a \refer{} set.
% \jbgcomment{don't use ``list'' unless it's ordered}
%
\abr{em} makes more sense in \emph{extractive} \abr{qa}, where the goal is to
find answers embedded in a fixed passage, but today it falters with models
that provide answers in different but correct forms.

% \paragraph{$F_1$ Score}
%
% \jbgcomment{if we're going to review F1, I think it's better to be a
%   little more precise.  What's a word?  Is it a space-delimited token,
%   a word piece a la the BERT tokenizer, or a lemma.  Perhaps an
%   example like ``King Charles III of England'' and ``King Louis III of
%   France'' would help clarify.  Then you could give the precision and
%   recall of this explicitly.  Perhaps something with initials would be
%   even more clarifying.}
%
% The $F_1$ score measures the token
% overlap between the \refer{} and \can{} answers, focusing on both precision and recall. Each continuous sequence of non-whitespace characters is a token. Suppose \refer{} answer \textit{\uline{World Health Organization global public health leader}} has 7 tokens--[\textit{"World", "Health", "Organization", "global", "public", "health", "leader"}], whereas \can{} answer \textit{\uline{WHO global leader}} has three tokens--[\textit{"WHO", "global", "leader"}]. Precision calculates the proportion of relevant words in the \can{} answer, while recall assesses the proportion of relevant words in the \refer{} answer that are also in the \can{} answer. The True Positive (\abr{tp}) between the examples are 2 since \textit{"global"} and \textit{"leader"}  are two common words in both answers; the False Positive (\abr{fp}) is 1 since \textit{"WHO"} is the token not present in the \refer{}; the False Negative (\abr{fn}) is 7 since there are 7 tokens in the \refer{} but not in the \can{}. Thus we calculate precision and recall using formulas:

% \begin{gather}
% \text{Precision} = \frac{\text{tp}}{\text{tp} + \text{fp}} \notag, 
% \text{Recall} = \frac{\text{tp}}{\text{tp} + \text{fn}} \notag
% \end{gather}
% The precision and recall are approximately 0.67 and 0.29, thus resulting $F_1$ score is 0.4. This method acknowledges the correctness of a \can{} answer
% by accessing essential information and amount of token overlap in the \refer{} answers, but does not take the context of the question into account. In addition,there is no consensus regarding the choice of threshold for $F_1$ score, making this metric more challenging to interpret than the \abr{em}. A 0.3 threshold will make the \can{} answer equivalent to the \refer{} but 0.5 will not. Section~\ref{section: classifier_training} will introduce how we combine $F_1$ with a new evaluation method, eliminating the need for threshold selection. 


\paragraph{Token Evaluation} 
%
Token $F_1$ score assess the precision and recall over the tokens in the 
the generated and \refer{} strings in token-level.
%
% Consider the question: \textit{\uline{Which organization is renowned for its leadership in addressing international health concerns and pandemics?}}  with reference \uline{World Health Organization global public health leader} and candidate \uline{WHO global leader}. The \can{} has three tokens [\textit{"WHO",
%   "global", "leader"}].  The \refer{} has seven.
%
$F_1$ counts how many tokens from \can{} are in the \refer{} (precision) and
how many of the \refer{} tokens were in the \can{} (recall) then takes the
harmonic mean of these number (exact details in
Appendix~\ref{appendix:F1_details}).
%
% \abr{bleu} score is originally used for machine translation and summarization evaluation, but can also be used to measure the similarity of the machine-generated text to one or more \refer{} texts, focusing on the precision of n-grams in the generated text compared to the \refer{} texts. BLEU scores are calculated for several n-gram lengths and combined into an overall score using a weighted average, emphasizing both the fluency and adequacy of the translation.
This produces a floating point number between 0.0 and 1.0 that encodes how
similar these sets of tokens are, but the challenge becomes knowing what
threshold is ``good enough''.
%
If a reference and candidate have 0.4 token $F_1$, a 0.3 threshold makes the \can{} answer
correct but 0.5 is incorrect.


\paragraph{Neural Evaluation}

Unlike string-based methods, \bertscore{}, \abr{bem}, and \abr{lerc} use
the knowledge and neural representations of models such as
\bert{}~\cite{devlin2018bert}.
%
\bertscore{} represents \can{}s and \refer{}s via a \abr{bert} representation
and computes the cosine similarity.
% \jbgcomment{check this, I edited to make it more precise, but didn't look it up to make sure it was correct}
%
\bem{} and \abr{lerc} use a trained \bert{} on human-annotated \ac{} and human rating examples, thus
providing a more fine-grained evaluation using context and world knowledge.
 
% \paragraph{\abr{bert}-Matching (\abr{bem})}
% \abr{bem} uses a \abr{bert}-based model trained on an \ac{} dataset
% that can can take the questions, \refer{}, and \can{} answers all
% into account to detect \can{} answer
% correctness.~\citep{bulian2022tomayto} provides two fundamental
% criteria to define \ac{} and annotate the \ac{} dataset based on
% %
% \textbf{1:} \can{} answers contain at least the same (or more)
% relevant information as the \refer{} answers, while taking into
% account of the context and the question; in particular it does not
% omit any relevant information present in the \refer{} answer should
% be ruled correct;
% \textbf{2:} \can{} answers contain neither
% misleading or excessive information not present in the \refer{}
% answers taking into account of the question and context should be
% ruled incorrect.
% %
% Fine-tuned \abr{bert}-based evaluation methods have the highest
% alignment with human judgments than \abr{em} and $F_1$ on their
% \ac{} test set.

%
% \jbgcomment{Non non-breaking space $(\verbatim{~})$ in front of citet}

% \citet{bulian2022tomayto} also contribute an \ac{} dataset derived from~\cite{rajpurkar2016squad}, which includes 23,260 \ac{} examples that contains crowd-sourced human annotated judgments on answer correctness, where each example contains the context for the question, the question, a \refer{} answer, a \can{} answer, and the human judgment of the \can{} answer.
% %
% Subsequently they split the dataset into train, dev and test set and trained a \abr{bert} matching (\abr{bem}) to assess \ac{}. \abr{bem} achieves the best alignment ($\textbf{89.66\%}$) with human judgment on the test set compared to $F_1$ ($75.95\%$), BertScore ($70.27\%$), and \abr{em} ($54.29\%$). However, the effectiveness of \abr{bem} on classifying answer correctness is only substantially evaluated on annotated datasets generated from SQuAD~\cite{rajpurkar2016squad}. \abr{bert}-based methods for classifying \ac{} and generalization for other variety of \abr{qa} problems remains unclear. Our hypothesis is that the alignment between human judgment and \abr{bert}-based \ac{} classification drops dramatically for out-of-distribution (\abr{ood}) \abr{qa} benchmark datasets, while standard evaluation metrics like \abr{em} continue to be highly misaligned with human correctness judgments. We explore the limitations of \abr{bem} and \abr{em} to classify \ac{} in the following section.

% Using this dataset, we analyze the alignment of \abr{bem} and \abr{em} with human judgments by evaluating their accuracy on the \ac{} dev and test set.~\footnote{We use a threthold of greater than 0.5 to judge an answer to be correct using \abr{bem} since \abr{bem} is trained with best performance with 0.5 threshold} In addition, we trained RoBERTa-base and LLAMA 2 on the \ac{} train set as additional automated correctness evaluation models to analyze the weaknesses of the definition of \ac{}, the \ac{} dataset, and the current automated evaluation models.~\footnote{Training details for RoBERTa-base and LLAMA 2 is in Appendix. We use LLAMA 2 with 7B parameter sizes}

% Table ~\ref{tab: google-ae-accuracy} shows that \abr{em} is least aligned with human correctness judgments. On the other hand,  \abr{bem}, RoBERTa, and LLAMA 2  highly correlate with human judgments. Though this is a positive feature, we are interested in testing whether \abr{llm}-based models still retain this alignment with human judgments on out-of-distribution (\abr{ood}) data. 

% \ishanicomment{Can we include some comments on how our metric can be easily incorporated to capture commonsense reasoning as raised by metareviewer? Can we do one more thing? Instead of a generic prompt, let us also experiment with chain-of-thought prompting for a few examples?}
\subsection{\abr{qa} Evaluation on Reasoning Data}
\label{section:generalization}

% \paragraph{Out-of-distribution (\abr{ood}) dataset}
We analyze errors on current \abr{qa} evaluation
methods using \abr{ropes}, which
focuses on causal situational reasoning in \abr{qa}~\cite{lin-etal-2019-reasoning}.
%
Each question has its context and a \refer{} answer. We use the \textit{dev}
set with 1,688 \abr{qa} pairs as our test set.
% \jbgcomment{``Situation'' passage sounds off to me.  ``Situational''?  ``Context''?}
%
% \jbgcomment{style checker should flag ``we conduct X'', we can usually be verbed ``We X''}
% \paragraph{\can{} answer generation}
%
We use \abr{flan-t5} \abr{xl}~\cite{flan-t5}, an instruction-tuned language
model to generate answers, concatenating background context to the question as
the prompt.\footnote{While T5 is no longer \abr{sota}, since our goal is
  distinguishing correct from incorrect answers, we only need a replicable
  model different from the extractive models to produce enough free-form
  answers.}
% \jbgcomment{It might be worthwhile to have a footnote that addresses why we're not using SOTA models for this.  Something like:
%   We acknowledge that this is no longer a \abt{sota} model, but since
%   our goal is distinguish correct from incorrect answers, our goal is
%   to have a relatively inexpensive model to run that is replicable
%   (e.g., other researchers can reproduce our results) and that is
%   ``creative'' (i.e., a generative \abr{lm}).
% }
% \paragraph{Pitfalls and generalization of current evaluation methods}
%
We manually judge and label 1,688 \can{} answers (Section~\ref{section:intro})
and compare
% \jbgcomment{rather than citing them all here again, you can use a backpointer to the previous section.} 
\abr{em},
$F_1$, \bertscore{} and \bem{}.\footnote{\abr{ropes} examples are easier compared to our later test sets.}

\paragraph{\abr{em} is overly strict}
%
\abr{em} considers 102 answers incorrect that 
are actually correct: 
% \abr{em} suffers when the
%\can{} answers are a good choice for the question but not in the
% \refer{} lists. 
e.g., \textit{\uline{12 PM} and \uline{12 noon}; \uline{Mount Everest}
  and \uline{Mt. Everest}; \uline{wetlands area} and \uline{wetland}} 
  % are all failure cases
% for \abr{em} to detect \ac{}. 
\abr{em} struggles with generative \abr{qa} and 
underestimates \abr{qa} models' accuracies.

% \jbgcomment{Need to use boldmath on F1}
\paragraph{\textbf{$F_1$} and \bertscore{} are sensitive to thresholding}
%
% \jbgcomment{you didn't discuss thresholding when introducing F1;
%   adding that example with a threshold would make this less
%   surprising}
%
We calculate token $F_1$ and \bertscore{}'s agreement with human judgment at
different thresholds.
%
We use $F_1$ with a threshold of 0.3 ($82\%$), 0.5
($96\%$), 0.7 ($94\%$), and \bertscore{} with 0.80 ($77\%$) and 0.95
($73\%$).\footnote{The numbers in parentheses after each threshold value is
  the percentage of examples that the metric agrees with humans. We choose a
  higher threshold value for \bertscore{} than token-based methods because
  \bertscore{} generates scores above 0.75 for most of the examples. We use
  \roberta{}-base.}
% $\F_1$ has the most agreement with human judgment at 0.5 ($94\%$) and the least agreement at 0.3 ($82\%$). 
% calculate the percentage of examples that align with human judgments (Table~\ref{tab:string_matching_threshold}). 
%
Typically the threshold is set uniformly for a dataset, but this can fail for
different answer styles, different cultural conventions (e.g., omitting
patronymics for Russian names).
%
For example \textit{``Will
  there be more or less blue ice at the glacier than the frozen over lake?''}
has the gold answer \uline{more} but would call \uline{more blue ice}
incorrect of the threshold were 0.5. Section~\ref{section: classifier_training} details the implementation of revised rules for assessing answer correctness in training a learned classifier. 
%
It addresses the limitations of fixed thresholds by introducing variable thresholds tailored to the specific rules used for evaluation.

% \begin{table}[t]
% \small
% \centering
% \begin{tabular}{ccccc}
% \hline
% \rowcolor{gray!50}
% Threshold & $F_1$ & \rougeone{} & \meteor{} \\ \hline
% 0.3 & 82.05 & 81.28 & 97.16  \\ 
% 0.5 & 96.98 & 95.97 & 64.57  \\ 
% 0.7 & 94.08 & 93.60 & 64.63  \\\hline
% \end{tabular}
% \caption{Agreement (\%) of human judgments and token-based evaluations using different thresholds. Although token-based evaluations sometimes agree with human judgments, the choice of threshold value depends on the dataset and \abr{qa} models.}
% \label{tab:string_matching_threshold}
% \end{table}


% \paragraph{\abr{bem} suffers on \abr{ood} datasets}
\paragraph{Neural evaluation cannot make sharp distinctions}
%
% \bertscore{} also turns similarity into a real number and thus also needs a threshold:\footnote{We choose a higher threshold value for \bertscore{} than token-based methods because \bertscore{} generates scores above 0.75 for most of the examples. We use \roberta{}-base as evaluation model.} 
% %
% we use 0.80 and 0.95.
% %
% These agreements are 77.67\% and 74.61\%.
%
We run \abr{bem} and \textit{Learned Evaluation metric for Reading Comprehension} \abr{lerc}~\cite{Chen_2020} on the test set by providing the question, \refer{} answer,
and \can{} answer for each example as evaluation. \abr{bem} has 58.41\% of human agreements and \abr{lerc} has 55.63\%.  
%
We analyze 100 disagreements from \bertscore{} (0.8) and 100 from \bem{}.\footnote{\abr{lerc} outputs a score rating from 1 to 5. We use threshold 4 throughout the paper to judge \ac{} based on \citet{Chen_2020}'s definition.}
%
% Although pre-trained representation language models can provide sentence semantic similarity between \refer{} and \can{} answers, 
%
About 70\% of the mistakes are due to the models' strong prior knowledge on
sentences, where \can{} answers are different but close in the embedding
space: \textit{\uline{more} and \uline{less}; \uline{Wednesday} and
  \uline{Thursday}; \uline{planet A} and \uline{planet B}; \uline{turn off}
  and \uline{on}} are all examples where human judges it as incorrect but
\abr{bem} and \bertscore{} judge as correct.
%
% Current \abr{bert} evaluation methods face challenges in generalization to out-of-distribution (\abr{ood}) test data.
\bem{} is trained with human annotated SQuAD~\cite{rajpurkar2016squad} \ac{}
dataset and disagrees with humans on data not
similar to the training set.
%

Popular \abr{qa} evaluations either fail on strict string and token matching or making clear distinctions between similar strings. We bridge the gap
between human and automatic evaluation by adopting professional human
evaluation rules and evaluate on seven automatic metrics and eight \abr{qa} datasets that include long-form answers.
% for its \ac{} training data
% with less -well-defined correctness rules and restrictions.

% % \jbgcomment{What's the ``middle part''?}
% Although the current \abr{qa} evaluations work okay in most of easy cases (the given answer is in the \refer{} answer set), there are still issues between human
% correctness decision making process and the current evaluation
% methods.
%
% New evaluation methods adopted from expert human decision
% process are needed in the current era of machine \abr{qa}.

% \ishanicomment{Can we make this table single column? This should save some space? Something like I did now?}


% \begin{table}[t] % This specifies that the table should appear at the top of the page
% \centering
% \tiny
% \renewcommand{\arraystretch}{1.5} % Increase row spacing
% \begin{tabular}{p{2cm}p{4.8cm}} % Adjust the column widths to fit one column of the page
% \hline
% \textbf{Rule} & \textbf{Description} \\ \hline
% $R_1$: Entity-aliasing & Widely recognized aliases, pseudonyms that are commonly associated with referred answer entities are acceptable. \\ 
% $R_2$: Numerical information & Exact dates, years, numerical values are required unless the question specifically asks for approximations. \\ 
% $R_3$: Less details & The answer provides less detail but should include the essential and correct information required by the question (specificity level 1). \\
% $R_4$: More details & The answer contains additional information that does not contradict the question or initial answer (specificity level 2). \\
% $R_5$: Semantic equivalence & A high degree of word overlap does not establish equivalence. The answer must be contextually and semantically accurate. \\
% $R_6$: Irrelevant information & Any irrelevant or inaccurate description related to the question should be considered incorrect. \\
% $R_7$: Other possible answers & The response is correct but not in the initially provided list. \\
% \hline
% \end{tabular}
% \caption{The correctness of a \can{} answer can be traced and categorized to
%   one or more of the above rules. We adopt the rules from \abr{naqt} modified
%   after analysis of an annotated dataset with human correctness judgments
%   between \refer{} answers and machine generated answers. The acceptability of
%   \abr{qa} model answers are based on these guidelines. Rules with
%   examples are in Table~\ref{tab:more_ae_examples} (Appendix).}

% % \ishanicomment{In order to justify the adoption of these rules, we can also provide examples and a very short description of the rules, as was done by the Tomahto, Tomato paper? Something like your Figure 1 in Appendix}
% \label{tab:guidelines}
% \end{table}





% We present the number of false negative (\abr{fn}) and false positive (\abr{fp}) between human gold labels and \abr{bem}, \abr{em} in Table ~\ref{fig:demo} to investigate failure modes of current evaluation methods. Even if \abr{bem} is improved based on Bertscore~\cite{Zhang2019BERTScoreET}, which also better aligns with human correctness judgment for in-distribution \ac{} test dataset, but it has a significant misalignment between human \ac{} judgments on unseen datasets- 702 misalignments. On the other hand, \abr{em} shows its usual disadvantage of not able to take semantic equivalence between the \can{} and \refer{} answer into account, resulting in 102 false negative misalignments. Although $F_1$ score results in the least number of total \abr{fp} and \abr{fn} counts in our \abr{ood} dataset, it does not take into the semantic information of the question and answers into account, and the $F_1$ score threshold value to determine \ac{} is ambiguous for different datasets. 

% \begin{table}[ht]
% % \small
% \centering
% \begin{tabular}{ccc}
% \hline
%  & \abr{em} & \abr{bem} \\ \hline
% \abr{fp} & 0 & 686 \\ 
% \abr{fn} & 102 & 16 \\ \hline
% \end{tabular}
% \caption{\abr{fp} occurs when the gold label is incorrect, but the evaluation method classifies it as correct; \abr{fn} occurs when the gold label is correct, but the evaluation method classifies it as incorrect. We show the number of \abr{fp} and \abr{fn} for \abr{em} and \abr{bem} compared to gold correctness. While \abr{em} has the problem of being too strict, often classifies potential correct \can{} answers as incorrect, \abr{bem} significantly fails on being too generous to classify incorrect \can{} answers on an \abr{ood} dataset.}
% \label{tab: error_count}
% \end{table}



% \begin{figure*}[!t]
%     \centering
%     \includegraphics[scale=0.25]{figures/pipeline1.pdf}
%     \caption{We use GPT-4 to generate \ac{} training examples based on our correctness guidelines. Our goal is this step is not to come up creative or tricky examples that can even trick a human. The purpose of expanding the seed examples is to improve \abr{bert}-based classification models' ability to evaluate correctness that align with our rules.}
%     \label{fig:framework}
%     % \ishani{Ishani: Can we explain here how we came up with the rules that we use as a prompt to GPT-4?}
% \end{figure*}



% We then run \abr{em}, \abr{bem}, finetuned-RoBERTa, and finetuned-LLAMA 2 evaluations to judge the correctness of answers. Results are shown in table ~\ref{tab:results}. We observe a wide gap between accuracy judgments among the four evaluation methods. \abr{bem} have the highest correctness accuracy judgments among the four metrics while \abr{em} is the lowest. We conduct an error analysis to analyze examples where there are disagreements among the four metrics. 




% using one benchmark dataset with its respective descriptions below. 
% We also run correctness evaluations on four benchmark \abr{qa} datasets to validate our hypothesis of \abr{bem} and RoBERTa's correctness judgment performance for \abr{ood} datasets. We describe our datasets given examples in table ~\ref{tab:dataset}

% \textbf{\abr{nq-open}} The Natural Questions Open dataset is an adoptation of the original Natural Questions dataset developed by ~\cite{kwiatkowski-etal-2019-natural}. 

% \textbf{\abr{Trivia\abr{qa}}} includes over 650,000 question-answer-evidence triples, sourced from trivia enthusiasts and online resources~\cite{joshi-etal-2017-triviaqa}. 

% \textbf{\abr{Narrative \abr{qa}}} is a Reading Comprehension dataset that provides narrative texts and requiring models to draw answers from the story context~\cite{kocisky-etal-2018-narrativeqa}. 

% \textbf{\abr{\abr{ropes}}} The Reading Comprehension with Commonsense Reasoning dataset focuses on situational reasoning in reading \abr{qa} pairs~\cite{lin-etal-2019-reasoning}. 


% \subsection{Error Analysis and Correctness Guidelines}
% We conduct error analysis on examples where those four metrics do not agree. Then we categorize the erroneous examples into $N$ general types. Relevant rules are also adopted and revised from \abr{naqt}. \zong{Expand how we derive the guidelines}




% \begin{table*}[ht]
% \small
% \begin{tabularx}{\textwidth}{
%    >{\hsize=0.6\hsize}X
%    >{\hsize=1.8\hsize}X
%    >{\hsize=0.9\hsize}X
%    >{\hsize=0.9\hsize}X
%    >{\hsize=0.8\hsize}X }
% \hline
% \rowcolor{gray!50}
% Rule & Description & Question & \refer{} & \can{} \\
% \hline
% % \rowcolor{neverchanging}
% entity-aliasing & Widely recognized aliases, pseudonyms, or alternative names that are commonly associated with the \refer{} answer entities are acceptable & who plays red on orange is new black & Kate Mulgrew & Katherine Maria Mulgrew/
% Correct \\
% \hline
% % \rowcolor{neverchanging}
% numerical-approximation & Exact numbers are required unless the context of the question allows for approximations or the answers allows approximations & What is the key number used to solve the ancient challenge of 'squaring the circle'? & pi & 3.14/Incorrect 
% \\
% \hline
% % % \rowcolor{slowchanging}
% time & Dates, years, centuries, and millennia should be exact. "71" is not acceptable for "1971." However, partial decades like "the fifties" refer to the most recently completed decade) & In which decade did the Korean War begin? & 1950s & the fifties/
% Correct\\
% \hline
% % % \rowcolor{slowchanging}
% singular and plural form & Both the singular and plural forms of non-specific nouns (e.g., "electron(s)," "river(s)") are typically acceptable. Using the plural form for specific nouns should be considered incorrect. & What is the name of Earth's natural satellite? & Earth’s Moon & Earth's Moons/
% Incorrect\\
% \hline
% % % \rowcolor{falsepremise}
% less details provided & If a \can{} answer provides less detail but includes the essential and correct information required by the question, it should be judged as correct. & What did Martin Luther King Jr. do to combat racial inequality? & He led the Civil Rights Movement & Civil Rights Movement/
% Correct\\
% \hline
% % % \rowcolor{falsepremise}
% more details provided &  \can{} answer contains the \refer{} answer or an equivalent part. The additional information must be factually correct and does not contradict the question or \refer{} answer. & What is the largest planet in our solar system? & Jupiter & The closest planet to the Sun is Jupiter/
% Correct\\
% \hline
% % % \rowcolor{falsepremise}
% semantic and token overlap &  A high degree of word overlap or similarity does not establish correctness. The answer must be contextually and factually accurate & Who was the sixth President of the United States, serving from 1825 to 1829 & John Quincy Adams & John Adams/
% Incorrect\\
% \hline
% irrelevant information & The \can{} answer is completely irrelevant to question and the given answer should be incorrect & What is the chemical formula for water? & H\textsubscript{2}O & Photosynthesis/
% Incorrect\\
% \hline
% \end{tabularx}
% \caption{A Comprehensive guideline to define correctness of answers, where the rules are adopted mainly from \abr{naqt} and slightly modified upon analysis of annotated dataset with human correctness judgments between \refer{} answers and machine generated answers. The acceptability of \abr{qa} model answers should be based on theses guidelines. Our correctness classification model is also trained to follow theses acceptability rules. \zong{Need to get better examples and also include incorrect answers.}}
% \label{tab: guidelines}
% \end{table*}


% \begin{table*}[ht]
% \small
% \centering
% \begin{tabular}{cccccccccc}
% \hline
% (Accuracy \%) & \abr{em} & \abr{bem} & RoBERTa & LLAMA 2 & \abr{bem}-aug & RoBERTa-aug & LLAMA 2-aug & Human\\ \hline
% \abr{nq-open} & 33.19 & 42.33 & 41.05 & 41.22 & 45.59 & 39.31 & 40.64 & ?\\ 
% Trivia\abr{qa} & ? & ? & ? & ? & ? & ? & ? & ? \\
% \abr{ropes} & 41.51 & 87.26 & 55.63 & 46.56 & 74.70 & 50.83 & 46.62 & ? \\
% Narrative-\abr{qa} & ? & ? & ? & ? & ? & ? & ? & ? \\
% \hline
% \end{tabular}
% \caption{The table shows the correctness evaluation using the four metrics. The metrics with `aug' indicates the models are trained with orginal \ac{} augmented training set with our additional generated \abr{qa} pairs that follow our correctness guidelines.}
% \label{tab:results}
% \end{table*}




% We start our information probing process by adopting and analyzing their dataset first based on four evaluation metrics- \abr{em}, \abr{bem}, LLAMA-2 7 billion(7B)~\cite{touvron2023llama} finetuned on their \ac{} training set, and provided human judgements. LLAMA-2 7B is a powerful open source large pre-trained language model that has comparable performance to black-box GPT-4 models that exhibit reasonable instruction following ability. We finetune LLAMA-2 7B to detect \ac{} as a proxy for GPT-4 for the first stage error analysis.~\footnote{We use Low Rank Adoptation~\cite{hu2021lora} to finetune on total 9090 \ac{} samples that have human judgements. We concatenate the question, \refer{} answer, and \can{} answer as input prompt, and human judgement label as output. We use epoch=5, learning rate=2$e^{-5}$, temperature=0.1, and batch size=4.} We use \abr{em}, \abr{bem}, and LLAMA-2 to evaluate the equivalence of \refer{} answers and \can{} answers on the test set (9724 examples). We then analyze pick the top 100 examples where \abr{em}, \abr{bem}, and LLAMA-2 do not agree. Table ~\ref{tab:error analysis} shows our initial error discoveries of the current \ac{} benchmark dataset. 

% \begin{table*}[h]
% \centering
% \begin{tabular}{c c c c c}
% \hline
% \refer{} & \can{} & \abr{bem} & Human Judgement & Category \\ \hline
% Planet A & Planet B & equivalent & not & similar strings \\ \hline
% Around 200-300 & 200-300 & equivalent & not & approximation \\ \hline
% It absorbs all the light & All the light & equivalent & not & wrong human judgement \\ \hline
% Peking & Beiping & not & equivalent & entity aliasing \\ \hline
% \end{tabular}
% \caption{The table shows problematic \abr{bem} or human judgement examples in the benchmark \ac{} dataset. We categorize the examples into finite set of categories.}
% \label{tab:error analysis}
% \end{table*}



==> sections/35-methology-old.tex <==
% \ishanicomment{'Low-resource' might be confusing, let us be specific and say 'Computationally Efficient'}
% \section{Low-Resource \abr{qa} Evaluation}
% \label{section: classifier_training}
% \begin{figure}[!t]
%     \makebox[\linewidth][c]{%
%         % \hspace{-0.5cm}  % Adjust X to the desired value
%         % \includegraphics[scale=0.28]{figures/new_pipeline.pdf}
%         \includegraphics[scale=0.7]{figures/ae_pipe.pdf}
%     }
%     % \caption{Using text input and raw token scores as features can help \cfm{} learn an optimal combination of $F_1$, precision, and recall score thresholds to judge different types of answers based on implicit learned rules.}
%     % \jbgcomment{If this could be compressed into one tall figure, it would save some whitespace}
%     \caption{Whenever exact match returns false between reference and candidate answers, we have a rule/type classifier that takes the question, reference, and candidate information and return a corresponding rule for the input, then we use the assigned classifier from a list of independent classifiers for each rule to judge the candidate answer.}

    
%     \label{fig:pipeline}
% \end{figure}


% \zongxiacomment{Give more details on the Method, providing pseudo code}


\abr{qa} evaluation is not a task like \abr{qa} where the size of the model is
a secondary consideration; an effective method (i.e., one that could be
adopted) needs to be accurate, fast, and low-cost.
%
This section's goal is to match the effectiveness of the \mm{} evaluation
while minimizing computation, latency, and disk space.
%
\abr{em}, and $F_1$ evaluations are fast and require no storage but are
superficial.
%
\mm{} evaluations are trainable, require substantial computation, disk space,
cost, computational time, and latency.
%
In aggregate, they are too expensive for universal adoption in standard
\abr{qa} training and evaluation pipelines.
%
% We want to not just build a system that does the best on \ac{} task but one that does the best with minimal resources because in training QA systems, it will be used many times. 


By revising \ac{} for machine \abr{qa}, we can construct an efficient
automatic evaluation that not only aligns with our \ac{} decision making
process, but also goes beyond token-level matching and competitive with \mm{}
semantic evaluations.

% jbg: Below paragraph was already covered in previous section
% 
% Token-level matching such as $F_1$ scores provides a score that contains rich information about the token overlap similarity between two sets of tokens, but the threshold for \ac{} can be very different for different types of questions and datasets. 
%
% Trained \bert{} semantic matching can measure the equivalence of two answers by taking the question and semantic similarity between \refer{} and \can{} answers into account, but its limitations are its strong prior knowledge that causes the model to generate high scores on similar type terms but have opposite meanings, and current \ac{} datasets that do not have fine-grained representative examples aligned with expert rules, and requirement of more computational resource than token matchings.

%
% \subsection{Improvement of Current Score-Based Evaluation Methods} 
% \label{section: classifier_training}

\paragraph{Representative training data construction}

We manually write five to ten representative \abr{qa} examples with human
judgments adopted and revised from our error analysis and the \abr{nqat} rule
book as seed examples.
%
Then we prompt \abr{gpt-4} with the rules and seed examples and ask it to
self-verify its generated judgment and rule type
classification~\cite{ren2023selfevaluation}.
%
We manually annotate 350 generated examples and end up with 3,989 \ac{}
examples.
%
We combine the 9,090 \ac{} training examples~\cite{bulian2022tomayto} and
1,688 annotated examples from \abr{ropes} \textit{dev} set with generated
examples as our \ac{}-augmented training set (exact details in
Appendix~\ref{sec:data_augmentation}).

\subsection{$F_1$ score and meta information as important features}

Although $F_1$ score, precision, and recall give superficial token-level
matching between the candidate and reference answers, they are not useless.
%
As we argue in the previous section, the specifics of a question can argue for
a higher or lower threshold.
%
This section argues how we use this and the guidelines summarized in
Table~\ref{tab:guidelines} can guide \ac{}.

% Depending on the question and \refer{}, they can help they play an important
% role as our features to determine which rule from  applies a
% given \abr{qa} example falls into, and what thresholds of these score
% combinations the model should use to judge the the correctness of an answer
% given a question falls into a rule type T(t), which will be further explained
% in the following sections.
% We follow the tokenization schemes in
% Section~\ref{sec:eval_methods} to treat words separated by space as a
% token. Appendix~\ref{appendix:F1_details} provides details for calculating the
% precision \textit{P}, recall \textit{R}, and $F_1$ scores between two strings.


\subsection{Question Rule Type Classifier}
% Each \abr{qa} example in our data includes the assigned \ac{} rule 1-7 in Table~\ref{tab:guidelines}. Specifically, a question \textit{Q} with a gold answer \textit{A}, for a candidate answer \textit{B}, we define the question type to be \textit{T} to fall in one of the seven answer categories when considering all three parts. We want to train a classifier such that given F(Q, A, B) = T(t), where T(t) is the mapping of the three question parts into one type of the rule.

\jbgcomment{This makes it sound like you have two classifiers, but what I
  think is happening is that you have two sets of features.  I think you need
  to say something like:


  - Set up the problem: map q, a, c -> T

  - We use a classifier to map examples.

  - This classifier has two features: an encoding of the text features and
  numeric features.

  - The encodings ...

  - The numeri features ...

}

Each \ac{} \abr{QA} example in our dataset corresponds to one of the seven
rules \( T\) defined in Table~\ref{tab:guidelines}.
%
Specifically, for a question \textit{Q} with a reference answer \textit{A},
and a candidate answer \textit{C}, we classify the question type \textit{T}.
%
% \textit{T} categorizes (Q, A, B) according to one of the predefined rules in the table~\ref{tab:guidelines}. 
%
Our objective is to train a classifier such that, given an encoding
\( E(Q, A, C) \), it predicts the rule type \( T(t) \), where \( T(t) \) maps the
combination of question, correct answer, and candidate answer to a specific
rule type. We use \textit{sklearn} count vectorizer to encode each example in
the input form of \textit{[CLS] \uline{candidate} [SEP] \uline{reference}
  [SEP] \uline{question} [SEP]}.
%
We then concatenate $F_1$, precision, and recall (floats) as additional
features with text encoding and train a logistic regression classifier to
classify \( T(t) \).\footnote{Training details in
  Appendix~\ref{sec:traing_hyperparameters}}
%
We define the classifier's output space for a given \abr{qa} example as
\(\textit{T(q)} = \{t_1, t_2, \ldots, t_7\}\), which is a vector containing
the probability of the \abr{QA} example being assigned to each rule.


\subsection{Contrastive Embedding Learning}

\abr{bert}-Tiny~\cite{turc2019} is a compact pretrained transformer model (18
MB) on large corpus of texts that can capture positional and semantic
relations between words.
%
It has two transformer layers with a hidden size of 128. We want to fully use
its positional embeddings to capture similarities and differences between
sentences in the semantic space.
%
To do so, we adopt ~\cite{1640964}'s contrastive loss to drive the learning of
embeddings by pushing apart dissimilar pairs while pulling together similar
pairs with the objective function:
{\small % This makes the text within the braces smaller
\begin{align}
L &= \frac{1}{N} \sum_{i=1}^{N} \bigg[ y_i \cdot (1 - \text{cos\_sim}_i) \nonumber \\
  &\quad + (1 - y_i) \cdot \max(0, \text{cos\_sim}_i - \theta) \bigg]
\label{eq:unified_contrastive_loss}
\end{align}
}
%
Where \(L\) represents the average loss calculated over all \(N\) pairs in the
dataset, \(y_i\) denotes the label of the \(i\)-th pair, \(1\) corresponds to
similar pairs and \(0\) to dissimilar pairs.
%
The term \(\text{cos\_sim}_i\) quantifies the cosine similarity between the
embeddings of the \(i\)-th pair.
%
The \(\text{max}(0, \text{cos\_sim}_i - \theta)\) component imposes a penalty
if the cosine similarity of a dissimilar pair exceeds the margin \(\theta\),
ensuring that dissimilar pairs are adequately distanced in the embedding
space.\footnote{We use $\theta$=0.8 since it gives us the highest accuracy on
  the \ac{} test set.}

%
For each \abr{qa} training pair, we treat pairs where candidate answers are labeled \textit{correct} as positive examples, and candidate answers that are labeled \textit{incorrect} as negative examples. 
%
To use the semantic meaning of questions when evaluating \ac{}, we also encode the question (\textit{Q}) and its associated answers as input. 
%
Specifically, we construct embeddings for both the reference pair (\textit{Q-A}) and the candidate pair (\textit{Q-C}), with labels based on candidate answer's \textit{correctness}. 
%
These embeddings are generated by encoding the sequences \textit{[CLS] \uline{candidate} [SEP] \uline{question} [SEP]} for (\textit{Q-A}) and \textit{[CLS] \uline{reference} [SEP] \uline{question} [SEP]} for (\textit{Q-C}). 
%
We then fine-tune \abr{bert}-Tiny using objective~\ref{eq:unified_contrastive_loss} to optimize the distance between the embeddings of (\textit{Q-A}) and (\textit{Q-C}) with hyperparameter details in Appendix~\ref{sec:traing_hyperparameters}. 
%
We use the output embeddings as semantic features for our following \ac{} classification, where we define as \textit{Contrastive(q)}.


% \abr{bert}-Tiny~\cite{turc2019} is a pretrained compact transformer-based model (18 MB) on large corpus of texts that can capture positional and semantic relations between words. It has 2 transformer layers with a hidden size of 128. We take this as an advantage, to fully use its positional embeddings to capture similarities and differences between words in the semantic space. To do so, we adopt ~\cite{1640964}'s contrastive loss to drive the learning of embeddings by pushing apart dissimilar pairs more than a margin while pulling together similar pairs. Specifically, we for each \abr{qa} example, pair, we treat the positive example pairs where candidate answers are labeled \textit{correct} as positive examples, where candidate answers that are labeled \textit{incorrect} as negative examples. 

% \paragraph{Going beyond exact match} Figure~\ref{fig:pipeline} shows how to have multiple classifiers to judge a candidate answer. If the candidate answer does not have an exact match with the reference answer, we use our trained classifier to determine the \ac{} rules applied to the given question, reference, and candidate. We train a classifier with \abr{qa} examples associated with each of the rules. Some rules require a more strict match between reference and candidate answers than others.

% shows how to combine advantages of token matching and semantic matching to train a classifier to learn an optimal combination of $F_1$, precision, and recall scores for different rules and answer types. For a classifier to learn such patterns, we first systematically construct representative example \abr{qa} pairs for each \ac{} rule, then train a classifier on the constructed set. 


%


% \paragraph{Feature Intuition} tf-idf~\cite{SprckJones2021ASI} encoding of the question, reference and candidate answers identifies which terms are important to answers (e.g., ``with'' and ``of'' are less important than ``Soviet'') and implicitly learn answer types from the question and answers, such as \textit{what, who, when}\dots 
%
% In addition, the classifier implicitly computes the cosine similarity between the reference and candidate answers to determine text similarity. 
%
% \paragraph{Individual classifier features} 
\subsection{Multi-Level Evaluation}
Section~\ref{sec:limitations} addresses one drawback of neural evaluations is that they tend to be affected by strong prior knowledge, where close words but different meanings easily produce a high similarity scores. 
%
To combat this issue, we also consider to use tf-idf~\cite{SprckJones2021ASI} encodings of the question, reference and candidate answers identifies which terms are important to answers (e.g., ``with'' and ``of'' are less important than ``Soviet'') and learn to rely more on word importance and token-level matching for specific rules, such as numerical answers that require a more strict matching.
%
We follow the \abr{bert}-matching encoding format to include separators between the question, reference and candidate answers: \textit{[CLS] \uline{\can{}} [SEP] \uline{\refer{}} [SEP] question [SEP]} for ease of human readiness, and use tf-idf to convert text to feature vectors. 
%
Then we compute the $F_1$ score, precision, and recall between \refer{} and \can{}; we concatenate the scores as float vectors to the encoded unigram text features: \textit{[CLS] \uline{Sep, 1945} [SEP] \uline{Sep 2, 1945} [SEP] What date did World War II end? [SEP] [0.8, 0.67, 1.0]}, where we define as \textit{IDF(q)}.
%
Under different \ac{} rules, the importance and combination of $F_1$, precision, and recall scores are different, and we want to train a model to learn such optimal combinations.

\paragraph{When to use what features?} We do not want to fully rely just on neural embeddings nor tf-idf embeddings to judge \ac{} for all rules. Rather, we want to take advantage on both methods that can be best suit for the type of the rule the question and answers fall into. 
%
Thus, given a question, a reference answer, and a candidate answer, we include \abr{bert}-Tiny's embeddings \textit{Contrastive(q)}, the tf-idf embedding \textit{IDF(q)}, and the rule type probability vector \textit{T(q)} from the rule-type classifier as features concatenated in the form \textit{[Contrastive(q), T(q), IDF(q)]} to train a classifier to judge a candidate answer's correctness.
%
Specifically, we use XGBoost~\cite{10.1145/2939672.2939785} to learn the non-linear relationships between the three concatenated features with hyperparameter details in Appendix~\ref{sec:traing_hyperparameters}.
%
Such classifier is not only able to take the advantage of semantic word relations from the \abr{bert} embeddings, but also benefit from maximally judge the correctness of an answer based on pre-defined rule types, and token overlap information.
%
\cfm{} is most effective for datasets with well-defined rules (Appendix~\ref{sec:unstructured_augmentation_experiment}).\footnote{We also experiment on augmented training set without well-defined rules, the resulting classifier is not well-aligned (Appendix~\ref{sec:unstructured_augmentation_experiment}).}
% %
% We follow the \abr{bert}-matching encoding format to include separators between the question, reference and candidate answers: \textit{[CLS] \uline{\can{}} [SEP] \uline{\refer{}} [SEP] question [SEP]}. Then we compute the $F_1$ score, precision, and recall between \refer{} and \can{}; we concatenate the scores to the encoded unigram text features: \textit{[CLS] \uline{Sep, 1945} [SEP] \uline{Sep 2, 1945} [SEP] What date did World War II end? [SEP] [0.8, 0.67, 1.0]}.
% % \jbgcomment{I thought we were underlining answers, not questions}
% \paragraph{Rule classifier features}
% % We also prompt \abr{gpt}-4 with associated \abr{ac} rules to judge each generated answer.
% Each \abr{qa} example in our data also includes the associated \ac{} rules to judge the answer. We then train a classifier to identify the rules of a \abr{qa} example. We use the same features as the individual classifier features to encode the input text and the rule as the output.
% \begin{enumerate}
%     \item \textit{[CLS] \uline{The currency in South Korea is called the South Korean Won} [SEP] \uline{Won} [SEP] What is the money called in South Korea? [SEP] [0.20, 1.0, 0.11]}
%     \item \textit{[CLS] \uline{Sep, 1945} [SEP] \uline{Sep 2, 1945} [SEP] What date did World War II end? [SEP] [0.8, 0.67, 1.0]}
% \end{enumerate}

%
%

% \textbf{The classifier automatically learns to capture semantic information from \abr{qa} pairs while also learns optimal explicit token overlap score threshold decision for different answer types}. 
% \jbgcomment{If it's easy to swap out, it might be worthwhile to try boosted decision trees or something like that; sometimes higher accuracy.  I expect it won't be better, but you could say in a footnote (XBoost was no better, so we retained LR for its interpretability).}

% \paragraph{Classifier Selection} We use logistic regression for its simplicity and efficiency. Additionally, we use \roberta{}-base as our comparison model and train on the original and our augmented \ac{} dataset following \citet{bulian2022tomayto}'s training format.~\footnote{We also used XGBoost decision tree and it was no better than logistic regression (\abr{lr}) classifier in our case~\cite{Chen_2016}, and we trained \abr{lr} for its efficiency}
%
% Theoretically, our base classifier does not have maximum
% input token length limit like \mm{}s do (usually 512 tokens), we can
% encode arbitrary length of text inputs including context as features,
% but this will not be in the scope of this paper.

%
% Among the constructed examples, we follow the human thought process to divide the questions into different types- \textit{what, who, when, where, how}, and the types of answers are determined by the questions and answers. 
%
% For each question and answer types, we have a different threshold to measure \ac{}. 
%
% For example, although \uline{DMV} and \uline{Department of Motor Vehicles} have no token overlap, they are referring to \textit{what} type, and the entity-aliasing rule. 
%
% Thus we still want to consider them equivalent even token-level matching has score 0. 
%
% When more details are provided, where the extra information will lower the token overlapping score using token-matching methods, and we want to have a lower $F_1$ score threshold to determine answer correctness.

%
% When questions and answers are numerical information, our rules state that numerical answers should be exact in most cases. Thus we want to have a higher $F_1$ score threshold to determine \ac{} for \abr{qa} pairs asking about numerical information. 
%
% An example is \textit{\uline{Sep 1945} and \uline{1945}}, although the $F_1$ score is 0.67, we want to set a higher $F_1$ score that for the type of answers for numerical information such that the \can{} answer is incorrect. The choice of token-matching threshold can vary based different types of questions and answers, which also requires an understanding of the question to determine the type of answer it is asking for.
%
% A classifier can mimic the human decision making process: first determine question and answer types with encoded texts, and assign them under a specific rule category implicitly; based on the question, \refer{} and \can{} answers, humans can determine the correctness of the \can{} answer by how much the \can{} answer overlaps with the \refer{} answer.
%



% The way we mimic the human judgment process to  to machine learning is that we can first construct a set of rules to correctness judgment, with many representative \abr{qa} pairs for each rule. There is a corresponding $F_1$ score indicating the token similarity and overlapping information for each \abr{qa} pair with \refer{} and \can{} answers.
%
% Our goal is to train a classifier that can take the \abr{qa} pairs as inputs to determine the type of answers the question is asking, then we also want the classifier take the $F_1$ score, precision, recall information between the \refer{} and \can{} answers and correlates with the answer types and contexts of the questions. 
%
% The classifier then learns an optimal $F_1$ token similarity threshold for each rule and answer type so when we use the classifier to judge a \can{} answer, the classifier first looks the the answer type based on the encoded text, then looks at the given token similarity information to judge correctness based on its learned optimal $F_1$ threshold from the training data.
%
% We have a pipeline process to mimic the human thought process of judgment, we delve into our training example data augmentation and classifier training details in the rest of this section. 






% \paragraph{Entity Aliasing Expansion}
% %
% This method is specifically targeted to correctness rule 1, where the
% \refer{} and \can{} answers are entities that have other possible
% aliases not in the current answer set.
% %
% This step is for users who wish
% a more rigorous evaluation that can find more relevant and timely
% aliasing entities from Wikipedia to increase the chance of answer
% matching depending on their model deployment and usage purposes. For
% example, if the evaluation dataset is constructed in 2016, where the
% \refer{} answer is only \textit{Burj Khalifa}, but when the question
% \textit{What is the tallest building in the world?} is asked today,
% the same building is also known for other aliasing names such as
% \textit{Khalifa Tower, Burj Dubai}.
% %
% In addition, a classifier trained on a fixed
% \ac{} dataset without updates of aliasing examples would also be a
% challenge to detect more general \ac{}.
% %
% Thus, we also include
% Wikipedia entity linking features~\cite{wikidata_pywikibot} into our
% evaluation pipeline to expand the \refer{} and \can{} answer set
% of our test sets if possible to improve \ac{} generalization, but
% this step can be turned on or off depending on users' purposes and
% trade off of more resource required.\footnote{This method is likely
% the most effective for datasets like TriviaQA, entityQ, HotpotQA,
% where many of the answers to questions are entities that have aliasing
% from the Wikipedia page, and is less effective for datasets like
% \abr{ropes}, where the answers are mainly based on context and
% reasoning of the questions.}

% Merely augmenting the training data for a classifier do not solve the
% entity aliasing issues, since there are many possible aliases to the
% same entity, and some of them will change over
% time. \citet{answerExpansion} show expanding the answer set can
% improve \abr{em}'s accuracy during evaluation step.  \jbgcomment{Give
%   example here, perhaps as part of a figure that shows the evolution
%   of the prompt through these steps in this subsection}
% %
% We also add
% Wikipedia entity linking to add into our evaluation pipeline. Given a
% \refer{} and a \can{} answer, we first use Wiki entity linking to
% expand the \refer{} and \can{} answer set if possible. If the
% expanded \refer{} and \can{} answer lists have an exact match, we
% determine the answers as equivalent.\footnote{This method is the most
% effective for datasets like TriviaQA, entityQ, PopQA, where many of
% the answers to questions are entities that have aliasing from the
% Wikipedia page, and is less effective for datasets like \abr{ropes},
% where the answers are mainly based on context and reasoning of the
% questions.}
%
% \jbgcomment{This sentence is unclear.  Does what you do solve the problem for all entities, some entities, etc.}
% Since this feature is only available when with internet access and is
% expensive to make \abr{api} queries to Wikipedia, we generate another
% set of evaluation data that expands the \refer{} answer set and
% generated \can{} answers generated from our test \abr{qa} models.


% \begin{table*}[ht]
% \centering
% \small
% \begin{tabular}{m{0.13\textwidth} m{0.08\textwidth} m{0.37\textwidth} m{0.16\textwidth} m{0.14\textwidth}}
% \hline
% \textbf{Dataset} & \textbf{\# Pairs} & \textbf{Context} & \textbf{Question} & \textbf{Gold Answer} \\ \hline
% % \abr{\abr{ropes}} & 1,688 & Michael Paul Welch (born August 25, 1972) is a former right-handed pitcher ...  was named a 2014 "Best High School" by U.S. News and World Report. & Mike Welch attended high school that serves how many students ? & 2,200 students \\ \hline
% \abr{nq-open} & 3,610 & \multicolumn{1}{c}{-} & who won the American league east in 2017 & The Yankees, Houston Astros \\ \hline 
% Hotpot\abr{qa} & 3,300 & Asmara International Airport (IATA: ASM) (ICAO: HHAS). Asmara currently hosts the country's only operating international airport... & Asmara international airport is in which country? & Eritrea \\ \hline
% Narrative-\abr{qa} & 3,300 & The narrator, a Bostonian, returns after a brief visit a few summers prior, to the small coastal town ... cMaine coastal town increases each day. & What was Littlepage's job? & sailor, retired sailor \\ 
% % \hline
% % \textit{Jeopardy}{}! & 371 & \multicolumn{1}{c}{-} & During the war, this Ozark state had 2 competing governments? & Arkansas \\ 
% \hline
% \end{tabular}
% \caption{The three datasets we use for our generalization testing. We do not include contexts for \abr{nq-open} for more variability of generated answers to challenge the evaluation methods. 
% % The \textit{Jeopardy}{}! dataset also includes the expert human responses and judgments of correctness.
% }


% % \caption{Number of \abr{qa} pair examples and datasets we use in our study to evaluate automated \abr{qa} evaluation metrics. The cell with `-' indicates the \abr{qa} pairs do not have related contexts.}

% \label{tab:dataset}
% \end{table*}


% \subsection{New Metric Construction}
% \subsection{Feature Engineering and Classifier Training}
% \label{section: classifier_training}
% \jbgcomment{I think you need to do a little more explanation of why you're trying these different models: we want to not just build a system that does the best on this task but one that does the best with minimal resources (latency, bandwidth, cost) because in training QA systems, it will be used many times.  Then remind the user that you're going to compare them.}

% To ensure the effectiveness of both our augmented training dataset,
% entity aliasing expansion method, and our small classifier to
% determine \ac{}, we conduct a three-way comparison validation
% experiment.

% \jbgcomment{Below paragraph needs clearer topic sentence.  Perhaps
  % something like: ``\equivalence{} is not a task like question
  % answering where the size of the model is a secondary consideration;
  % rather, an effective method (i.e., that could be adopted) needs to
  % be efficient as well.  The goal of this section is to match the
  % effectiveness of the prior \abr{gpt}-based method while also
  % minimizing computation, latency, and disk space.''}



% \paragraph{Classifier Selection} We use logistic regression (\abr{lr}) as our base classifier for its simplicity and efficiency. Additionally, we use \roberta{}-base as our comparison model and train on the original and our augmented \ac{} dataset following \citet{bulian2022tomayto}'s training format.

% \jbgcomment{I think we need a word or two about the intuition of why we need tf-idf, what's an example of where that could help?}

% \paragraph{Feature selection} tf-idf~\cite{SprckJones2021ASI} transforms texts into numerical representation and measures how frequent a term appears in the input text and how important the term is across all the training data. 
% %
% Thus we use tf-idf unigram to encode the question, reference and candidate answers, where the classifier can possibly detect answer types from the question and answers, such as \textit{what, who, when}\dots 
% %
% In addition, the classifier implicitly computes the cosine similarity between the reference and candidate answers to determine text similarity. 
% %
% Paired with implicit cosine similarity and question context, we also concatenate the encoded text features with $F_1$ score, precision, and recall that provides explicit token-overlap information between answers to learn an optimal threshold for different answer types and different cosine similarity. This technique is the most effective for \ac{} dataset with well-defined rules as shown in Section~\ref{sec:metric_comparison}.\\
% %
% We follow \abr{bert}-matching encoding format to include explicit separators between the question, reference and candidate answers: \textit{[CLS] \uline{\can{}} [SEP] \uline{\refer{}} [SEP] question [SEP]}, where an encoding vectorizer will encode the \textit{[CLS]} and \textit{[SEP]} tokens as separator between questions and answers. In addition, we compute the $F_1$ score, precision, and recall for each \refer{} and \can{} pair; we concatenate the $F_1$ score, precision and recall to the encoded unigram text features as inputs to our base classifier. We show examples visualizations of \abr{qa} pairs turned into features:
% \begin{enumerate}
%     \item \textit{[CLS] \uline{The currency in South Korea is called the South Korean Won} [SEP] \uline{Won} [SEP] What is the money called in South Korea? [SEP] [0.20, 1.0, 0.11]}
%     \item \textit{[CLS] \uline{Sep, 1945} [SEP] \uline{Sep 2, 1945} [SEP] What date did World War II end? [SEP] [0.8, 0.67, 1.0]}
% \end{enumerate}
% \textbf{The classifier automatically learns to capture semantic information from \abr{qa} pairs while also learns optimal explicit token overlap score threshold decision for different answer types}. Theoretically, our base classifier does not have maximum
% input token length limit like \mm{}s do (usually 512 tokens), we can
% encode arbitrary length of text inputs including context as features,
% but this will not be in the scope of this paper.


% \jbgcomment{I think the discussion of features can be a little longer, perhaps give an example of what 2-3 examples look like when turned into features}


% \subsection{Muppet Judge Training}
% To ensure the effectiveness of our augmented training curriculum materials and the generalization of them on different Muppet Judges, we use \abr{bert}-base-uncased, distil\abr{bert}-base-uncased, \abr{r}o\abr{bert}a, and distil\abr{r}o\abr{bert}a as our correctness classification model. We adopt the most effective training template from ~\cite{bulian2022tomayto} by concatenating the \can{} answers, \refer{} answers, and the questions together as: \textit{[CLS] \can{} [SEP] \refer{} [SEP] question [SEP]}. Then we train our selected Muppet Judges on the original \ac{} train set (except for \abr{bert}, which we will use \abr{bem} directly) and the rule-enforced augmented set.\footnote{We use a learning rate $1e^{-5}$, batch size 16, weight decay of 0.1 for 10 epochs. We save the state model with the highest \textit{dev} set accuracy. We set a threshold of above 0.5 as correct for a \can{} answer.} Subsequently, we use the Muppet Judges to evaluate \ac{} on two styles of benchmark and one challenge \abr{qa} dataset. The following section analyzes the improvement of our Muppet Judges with new training materials. 

% \begin{table*}[t]
% \centering
% % \footnotesize
% \scriptsize
% \setlength\tabcolsep{4.5pt} % Reduce space between columns
% % \small
% \begin{tabular}{cccccccccccc}
% \hline
% \rowcolor{gray!50}
% \textbf{Dataset} & \textbf{EM} & \textbf{$F_1$} & \textbf{BERTscore} & \textbf{ROBERTA} & \textbf{\cfm{}} & \textbf{LLaMA70B-Eval} & \textbf{GPT-4-Eval} & \textbf{QA Model} \\
% \hline
% \multirow{3}{*}{\textbf{\abr{nq-open}}} 
% & 0.76 & 0.74 & 0.26 & 0.47 & 0.73 & \textcolor{red!50}{86.39}/\textcolor{blue!50}{0.11} & 0.80 & Flan-T5 xl \\ 

% & 0.65 & 0.28 & 0.34 & 0.50 & 0.68 & \textcolor{red!50}{84.15}/\textcolor{blue!50}{0.06} & 0.77 & LLaMA 2 7B \\

% & 0.62 & 0.41 & 0.41 & 0.55 & 0.72 & \textcolor{red!50}{89.00}/\textcolor{blue!50}{0.07} & 0.77 & GPT-3.5-turbo  \\
% \hline

% \multirow{3}{*}{\textbf{NQA}} 
% & 0.33 & 0.43 & 0.20 & 0.58 & 0.49 & \textcolor{red!50}{88.64}/\textcolor{blue!50}{0.11} & 0.76 & Flan-T5 xl \\ 

% & 0.32 & 0.25 & 0.16 & 0.56 & 0.50 & \textcolor{red!50}{94.12}/\textcolor{blue!50}{0.06} & 0.74 & LLaMA 2 7B \\

% & 0.25 & 0.17 & 0.08 & 0.53 & 0.47 & \textcolor{red!50}{95.39}/\textcolor{blue!50}{0.07} & 0.78 & GPT-3.5-turbo \\
% \hline

% \multirow{3}{*}{\textbf{Hotpot \abr{qa}}}
% & 0.57 & 0.62 & 0.42 & 0.60 & 0.71 & \textcolor{red!50}{92.21}/\textcolor{blue!50}{0.11} & 0.78 & Flan-T5 xl \\ 

% & 0.66 & 0.48 & 0.40 & 0.65 & 0.75 & \textcolor{red!50}{83.93}/\textcolor{blue!50}{0.05} & 0.87 & LLaMA 2 7B \\ 

% & 0.60 & 0.47 & 0.37 & 0.62 & 0.75 & \textcolor{red!50}{89.93}/\textcolor{blue!50}{0.06} & 0.76 & GPT-3.5-turbo  \\
% \hline

% \multirow{3}{*}{\textbf{COQA}} 
% & 0.30 & 0.24 & 0.22 & 0.38 & 0.40 & \textcolor{red!50}{82.65}/\textcolor{blue!50}{0.37} & 0.65 & Mistral 8x7b  \\ 

% & 0.33 & 0.26 & 0.20 & 0.43 & 0.34 & \textcolor{red!50}{86.89}/\textcolor{blue!50}{0.09} & 0.80 & Yi-Chat 34B \\ 

% & 0.28 & 0.24 & 0.05 & 0.38 & 0.27 & \textcolor{red!50}{83.12}/\textcolor{blue!50}{0.02} & 0.80 & LLaMA2 70B  \\
% \hline

% \multirow{3}{*}{\textbf{BIOMRC}} 
% & 0.23 & 0.15 & 0.19 & 0.22 & 0.38 & \textcolor{red!50}{83.53}/\textcolor{blue!50}{0.40} & 0.70 & Mistral 8x7b  \\ 

% & 0.16 & 0.16 & 0.20 & 0.25 & 0.35 & \textcolor{red!50}{89.29}/\textcolor{blue!50}{0.05} & 0.80 & Yi-Chat 34B \\ 

% & 0.26 & 0.26 & 0.21 & 0.32 & 0.43 & \textcolor{red!50}{87.76}/\textcolor{blue!50}{0.02} & 0.79 & LLaMA2 70B \\
% \hline

% \multirow{3}{*}{\textbf{MS MARCO}} 
% & 0.22 & 0.10 & 0.20 & 0.22 & 0.33 & \textcolor{red!50}{82.30}/\textcolor{blue!50}{0.33} & 0.73 & Mistral 8x7b  \\ 

% & 0.25 & 0.11 & 0.15 & 0.19 & 0.33 & \textcolor{red!50}{88.43}/\textcolor{blue!50}{0.02} & 0.80 & Yi-Chat 34B \\ 

% & 0.27 & 0.24 & 0.22 & 0.36 & 0.45 & \textcolor{red!50}{87.00}/\textcolor{blue!50}{0.02} & 0.79 & LLaMA2 70B \\
% \hline

% \end{tabular}
% % \jbgcomment{Nice takeway, move the flip closer to the takeaway in the caption}
% \caption{We show each evaluation method's Pearson correlation with human judgments. \abr{em}, $F_1$, and \bertscore{} have unstable human agreement on different \abr{qa} datasets-- ranging from 0.10 to 0.76. \roberta{}, \cfm{} and \abr{gpt4}-Eval are more robust and stable with varying \abr{qa} datasets. Although LLaMA70B-Eval has constantly high agreement, it has high precision and low recall, and result in a low macro $F_1$. \cfm{} is less costly than \abr{gpt-4}, LLaMA70B, \roberta{}, and \bertscore{} and has more stable human agreements across six evaluation datasets than \abr{em}. \zongxiacomment{Really debating whether we should use human agreement percentage and Macro F1 or Pearson correlation. Pearson correlation is much lower than LLaMA70B-Eval, but not Macro F1 score.}}
% \label{tab:huamn_evaluation}
% \end{table*}


\begin{table*}[t]
\centering
% \footnotesize
\scriptsize
\setlength\tabcolsep{4.5pt} % Reduce space between columns
% \small
\begin{tabular}{cccccccccccc}
\hline
\rowcolor{gray!50}
\textbf{Dataset} & \textbf{EM} & \textbf{$F_1$} & \textbf{BERTscore} & \textbf{ROBERTA} & \textbf{\cfm{}} & \textbf{LLaMA70B-Eval} & \textbf{GPT-4-Eval} & \textbf{QA Model} \\
\hline
\multirow{3}{*}{\textbf{\abr{nq-open}}} 
& \textcolor{red!50}{89.38}/\textcolor{blue!50}{0.81} & \textcolor{red!50}{90.34}/\textcolor{blue!50}{0.82} & \textcolor{red!50}{50.40}/\textcolor{blue!50}{0.48} & \textcolor{red!50}{86.77}/\textcolor{blue!50}{0.79} & \textcolor{red!50}{92.76}/\textcolor{blue!50}{0.85} & \textcolor{red!50}{86.39}/\textcolor{blue!50}{0.11} & \textcolor{red!50}{96.69}/\textcolor{blue!50}{0.93} & Flan-T5 xl \\ 
& \textcolor{red!50}{82.21}/\textcolor{blue!50}{0.80} & \textcolor{red!50}{62.71}/\textcolor{blue!50}{0.50} & \textcolor{red!50}{66.43}/\textcolor{blue!50}{0.66} & \textcolor{red!50}{82.46}/\textcolor{blue!50}{0.81} & \textcolor{red!50}{84.13}/\textcolor{blue!50}{0.84} & \textcolor{red!50}{84.15}/\textcolor{blue!50}{0.06} & \textcolor{red!50}{93.48}/\textcolor{blue!50}{0.49} & LLaMA 2 7B \\
& \textcolor{red!50}{77.60}/\textcolor{blue!50}{0.76} & \textcolor{red!50}{58.85}/\textcolor{blue!50}{0.58} & \textcolor{red!50}{73.15}/\textcolor{blue!50}{0.68} & \textcolor{red!50}{90.63}/\textcolor{blue!50}{0.72} & \textcolor{red!50}{89.26}/\textcolor{blue!50}{0.74} & \textcolor{red!50}{89.00}/\textcolor{blue!50}{0.07} & \textcolor{red!50}{94.73}/\textcolor{blue!50}{0.95} & GPT-3.5-turbo  \\
\hline

\multirow{3}{*}{\textbf{NQA}} 
& \textcolor{red!50}{58.13}/\textcolor{blue!50}{0.50} & \textcolor{red!50}{77.19}/\textcolor{blue!50}{0.65} & \textcolor{red!50}{88.70}/\textcolor{blue!50}{0.57} & \textcolor{red!50}{83.62}/\textcolor{blue!50}{0.81} & \textcolor{red!50}{85.37}/\textcolor{blue!50}{0.84} & \textcolor{red!50}{88.64}/\textcolor{blue!50}{0.11} & \textcolor{red!50}{95.12}/\textcolor{blue!50}{0.97} & Flan-T5 xl \\ 
& \textcolor{red!50}{65.72}/\textcolor{blue!50}{0.54} & \textcolor{red!50}{52.53}/\textcolor{blue!50}{0.46} & \textcolor{red!50}{88.39}/\textcolor{blue!50}{0.54} & \textcolor{red!50}{91.66}/\textcolor{blue!50}{0.67} & \textcolor{red!50}{90.45}/\textcolor{blue!50}{0.76} & \textcolor{red!50}{94.12}/\textcolor{blue!50}{0.06} & \textcolor{red!50}{95.18}/\textcolor{blue!50}{0.49} & LLaMA 2 7B \\
& \textcolor{red!50}{64.81}/\textcolor{blue!50}{0.48} & \textcolor{red!50}{47.99}/\textcolor{blue!50}{0.38} & \textcolor{red!50}{91.84}/\textcolor{blue!50}{0.53} & \textcolor{red!50}{95.98}/\textcolor{blue!50}{0.66} & \textcolor{red!50}{92.24}/\textcolor{blue!50}{0.69} & \textcolor{red!50}{95.39}/\textcolor{blue!50}{0.07} & \textcolor{red!50}{97.33}/\textcolor{blue!50}{0.65} & GPT-3.5-turbo \\
\hline

\multirow{3}{*}{\textbf{Hotpot \abr{qa}}}
& \textcolor{red!50}{77.35}/\textcolor{blue!50}{0.71} & \textcolor{red!50}{85.87}/\textcolor{blue!50}{0.79} & \textcolor{red!50}{84.11}/\textcolor{blue!50}{0.70} & \textcolor{red!50}{86.94}/\textcolor{blue!50}{0.75} & \textcolor{red!50}{91.23}/\textcolor{blue!50}{0.85} & \textcolor{red!50}{92.21}/\textcolor{blue!50}{0.11} & \textcolor{red!50}{93.78}/\textcolor{blue!50}{0.91} & Flan-T5 xl \\ 
& \textcolor{red!50}{81.69}/\textcolor{blue!50}{0.81} & \textcolor{red!50}{66.51}/\textcolor{blue!50}{0.67} & \textcolor{red!50}{70.23}/\textcolor{blue!50}{0.67} & \textcolor{red!50}{80.02}/\textcolor{blue!50}{0.78} & \textcolor{red!50}{88.57}/\textcolor{blue!50}{0.88} & \textcolor{red!50}{83.93}/\textcolor{blue!50}{0.05} & \textcolor{red!50}{96.79}/\textcolor{blue!50}{0.49} & LLaMA 2 7B \\ 
& \textcolor{red!50}{79.68}/\textcolor{blue!50}{0.76} & \textcolor{red!50}{68.00}/\textcolor{blue!50}{0.66} & \textcolor{red!50}{76.23}/\textcolor{blue!50}{0.66} & \textcolor{red!50}{81.97}/\textcolor{blue!50}{0.76} & \textcolor{red!50}{90.50}/\textcolor{blue!50}{0.87} & \textcolor{red!50}{89.93}/\textcolor{blue!50}{0.06} & \textcolor{red!50}{93.87}/\textcolor{blue!50}{0.65} & GPT-3.5-turbo  \\
\hline

\multirow{3}{*}{\textbf{COQA}} 
& \textcolor{red!50}{74.82}/\textcolor{blue!50}{0.54} & \textcolor{red!50}{76.78}/\textcolor{blue!50}{0.52} & \textcolor{red!50}{47.45}/\textcolor{blue!50}{0.47} & \textcolor{red!50}{70.04}/\textcolor{blue!50}{0.62} & \textcolor{red!50}{77.60}/\textcolor{blue!50}{0.64} & \textcolor{red!50}{82.65}/\textcolor{blue!50}{0.37} & \textcolor{red!50}{87.56}/\textcolor{blue!50}{0.75} & Mistral 8x7b  \\ 
& \textcolor{red!50}{80.22}/\textcolor{blue!50}{0.57} & \textcolor{red!50}{79.26}/\textcolor{blue!50}{0.57} & \textcolor{red!50}{38.97}/\textcolor{blue!50}{0.39} & \textcolor{red!50}{69.53}/\textcolor{blue!50}{0.62} & \textcolor{red!50}{78.04}/\textcolor{blue!50}{0.65} & \textcolor{red!50}{86.89}/\textcolor{blue!50}{0.09} & \textcolor{red!50}{94.38}/\textcolor{blue!50}{0.86} & Yi-Chat 34B \\ 
& \textcolor{red!50}{78.44}/\textcolor{blue!50}{0.53} & \textcolor{red!50}{78.33}/\textcolor{blue!50}{0.55} & \textcolor{red!50}{36.14}/\textcolor{blue!50}{0.36} & \textcolor{red!50}{67.62}/\textcolor{blue!50}{0.59} & \textcolor{red!50}{78.42}/\textcolor{blue!50}{0.63} & \textcolor{red!50}{83.12}/\textcolor{blue!50}{0.02} & \textcolor{red!50}{90.81}/\textcolor{blue!50}{0.83} & LLaMA2 70B  \\
\hline

\multirow{3}{*}{\textbf{BIOMRC}} 
& \textcolor{red!50}{40.79}/\textcolor{blue!50}{0.39} & \textcolor{red!50}{27.31}/\textcolor{blue!50}{0.27} & \textcolor{red!50}{80.55}/\textcolor{blue!50}{0.58} & \textcolor{red!50}{88.71}/\textcolor{blue!50}{0.67} & \textcolor{red!50}{83.52}/\textcolor{blue!50}{0.67} & \textcolor{red!50}{83.53}/\textcolor{blue!50}{0.40} & \textcolor{red!50}{89.51}/\textcolor{blue!50}{0.86} & Mistral 8x7b  \\ 
& \textcolor{red!50}{42.97}/\textcolor{blue!50}{0.40} & \textcolor{red!50}{30.44}/\textcolor{blue!50}{0.30} & \textcolor{red!50}{79.53}/\textcolor{blue!50}{0.57} & \textcolor{red!50}{87.98}/\textcolor{blue!50}{0.67} & \textcolor{red!50}{82.67}/\textcolor{blue!50}{0.67} & \textcolor{red!50}{89.29}/\textcolor{blue!50}{0.05} & \textcolor{red!50}{88.71}/\textcolor{blue!50}{0.83} & Yi-Chat 34B \\ 
& \textcolor{red!50}{43.77}/\textcolor{blue!50}{0.42} & \textcolor{red!50}{50.55}/\textcolor{blue!50}{0.47} & \textcolor{red!50}{83.46}/\textcolor{blue!50}{0.59} & \textcolor{red!50}{84.04}/\textcolor{blue!50}{0.64} & \textcolor{red!50}{79.60}/\textcolor{blue!50}{0.68} & \textcolor{red!50}{87.76}/\textcolor{blue!50}{0.02} & \textcolor{red!50}{90.67}/\textcolor{blue!50}{0.87} & LLaMA2 70B \\
\hline

\multirow{3}{*}{\textbf{MS MARCO}} 
& \textcolor{red!50}{41.03}/\textcolor{blue!50}{0.39} & \textcolor{red!50}{25.40}/\textcolor{blue!50}{0.25} & \textcolor{red!50}{79.87}/\textcolor{blue!50}{0.58} & \textcolor{red!50}{88.53}/\textcolor{blue!50}{0.68} & \textcolor{red!50}{81.53}/\textcolor{blue!50}{0.65} & \textcolor{red!50}{82.30}/\textcolor{blue!50}{0.33} & \textcolor{red!50}{88.37}/\textcolor{blue!50}{0.88} & Mistral 8x7b  \\ 
& \textcolor{red!50}{42.67}/\textcolor{blue!50}{0.41} & \textcolor{red!50}{27.00}/\textcolor{blue!50}{0.27} & \textcolor{red!50}{78.27}/\textcolor{blue!50}{0.56} & \textcolor{red!50}{86.77}/\textcolor{blue!50}{0.64} & \textcolor{red!50}{80.77}/\textcolor{blue!50}{0.65} & \textcolor{red!50}{88.43}/\textcolor{blue!50}{0.02} & \textcolor{red!50}{87.57}/\textcolor{blue!50}{0.89} & Yi-Chat 34B \\ 
& \textcolor{red!50}{43.90}/\textcolor{blue!50}{0.43} & \textcolor{red!50}{48.63}/\textcolor{blue!50}{0.46} & \textcolor{red!50}{82.96}/\textcolor{blue!50}{0.59} & \textcolor{red!50}{84.13}/\textcolor{blue!50}{0.65} & \textcolor{red!50}{80.53}/\textcolor{blue!50}{0.68} & \textcolor{red!50}{87.00}/\textcolor{blue!50}{0.02} & \textcolor{red!50}{89.53}/\textcolor{blue!50}{0.90} & LLaMA2 70B \\
\hline

\end{tabular}
% \jbgcomment{Nice takeway, move the flip closer to the takeaway in the caption}
\caption{The red signifies human agreement ($\%$) and blue is the Macro $F_1$ score with human judgments. \abr{em}, $F_1$, and \bertscore{} have unstable human agreement on different \abr{qa} datasets-- ranging from $25\%$ to $90\%$. \roberta{}, \cfm{}, LLaMA70B-Eval and \abr{gpt4}-Eval are more robust and stable with varying \abr{qa} datasets. Although LLaMA70B-Eval has constantly high agreement, it has high precision and low recall, and result in a low macro $F_1$. \cfm{} is less costly than \abr{gpt-4}, LLaMA70B, \roberta{}, and \bertscore{} and has more stable human agreements across six evaluation datasets than \abr{em}. \zongxiacomment{Use Pearson Correlation}}
\label{tab:huamn_evaluation}
\end{table*}

